Competition and Anomalies Redux: Evidence from U.S. Auto Dealers

We examine a choice between bonus contracts offered to dealers of a U.S. auto manufacturer. In our data, dealers select the non-profit-maximizing option in 20 percent of observations, costing the mistaken dealers $18,453 per year on average. We examine how the propensity to make this mistake varies with competition, identified both cross-sectionally and within dealers over time. Both analyses show that greater competition substantially lowers the rate of mistakes. However, even in the most competitive markets, consequential mistakes persist. Our results suggest that competition disciplines mainly through within-dealer changes in behavior rather than entry and exit.

==> results/shr_high2017.tex <==
High tier&&0.163&\sym{***}& &&0.163&\sym{***}\\
&&(0.008&)&&&(0.008&)\\


==> results/shr_high2018.tex <==
High tier&&0.101&\sym{***}& &&0.101&\sym{***}\\
&&(0.006&)&&&(0.006&)\\


==> results/shr_high2019.tex <==
High tier&&0.091&\sym{***}& &&0.091&\sym{***}\\
&&(0.006&)&&&(0.006&)\\


==> results/shr_low2017.tex <==
Low tier&&0.025&\sym{***}&0.025&\sym{***}& &\\
&&(0.003&)&(0.003&)&&\\


==> results/shr_low2018.tex <==
Low tier&&0.000&&0.000&& &\\
&&&&&&&\\


==> results/shr_low2019.tex <==
Low tier&&0.000&&0.000&& &\\
&&&&&&&\\


==> results/shr_mistake2017.tex <==
Not ex-post max.&&0.236&\sym{***}&0.038&\sym{***}&0.197&\sym{***}\\
&&(0.009&)&(0.004&)&(0.008&)\\


==> results/shr_mistake2018.tex <==
Not ex-post max.&&0.203&\sym{***}&0.052&\sym{***}&0.151&\sym{***}\\
&&(0.008&)&(0.005&)&(0.007&)\\


==> results/shr_mistake2019.tex <==
Not ex-post max.&&0.161&\sym{***}&0.036&\sym{***}&0.125&\sym{***}\\
&&(0.008&)&(0.004&)&(0.007&)\\


==> results/shr_mistake_N2017.tex <==
\(N\) (dealerships)&&2,345&&2,345&&2,345&\\


==> results/shr_mistake_N2018.tex <==
\(N\) (dealerships)&&2,336&&2,336&&2,336&\\


==> results/shr_mistake_N2019.tex <==
\(N\) (dealerships)&&2,174&&2,174&&2,174&\\


==> results/shr_noenroll2017.tex <==
No enroll&&0.048&\sym{***}&0.013&\sym{***}&0.035&\sym{***}\\
&&(0.004&)&(0.002&)&(0.004&)\\


==> results/shr_noenroll2018.tex <==
No enroll&&0.102&\sym{***}&0.052&\sym{***}&0.050&\sym{***}\\
&&(0.006&)&(0.005&)&(0.005&)\\


==> results/shr_noenroll2019.tex <==
No enroll&&0.070&\sym{***}&0.036&\sym{***}&0.034&\sym{***}\\
&&(0.005&)&(0.004&)&(0.004&)\\

